Study of Baryon number transport using model simulations in $pp$ collisions at LHC Energies

We report on the excitation function of anti-baryon to baryon ratios ($\overline{p}/p$, {\alam /\lam} and {\axi / \xim}) in $pp$ collisions at {\sqrts} = 0.9, 2.76, 7 TeV from DPMJET-III, Pythia~8, EPOS~1.99, and EPOS-LHC model simulations. To study the predictions of these models at {\sqrts} = 13.6 TeV. The anti-baryon to baryon ratios are extremely important for the study of baryon number transport mechanisms. These ratios help determine the carriers of the baryon number and in the extraction of baryon structure information. Even though all models show a good agreement between model simulations and data, the ratios extracted from DPMJET-III model closely describes data at all energies. It is observed that these ratios converge to unity for various model predictions. This convergence also indicates that the anti-baryon to baryon ratios follow the mass hierarchy, such that the hyperon specie containing more strange quarks ({\alam /\lam} and {\axi / \xim}) approaches unity faster than specie containing fewer strange quarks ($\overline{p}/p$). It is also observed that the $\overline{B}/B$ ratio approaches unity more rapidly with the increase in {\sqrts} energy. At lower energies we observe an excess production of baryons over anti-baryons. However, this effect vanishes at higher energies due to the baryon-anti-baryon pair production and the baryon-anti-baryon yield becomes equal. Using model simulations, we additionally compute the asymmetry, ($A\equiv\frac{N_{p}-N_{\bar{p}}}N_{p}+N_{\bar{p}}}$) for protons. The asymmetry shows a decreasing trend with increase in energy from 0.9 to 7 TeV for all energies. This asymmetry trend is confirmed by model predictions at {\sqrts} = 13.6 TeV which will help to put possible constraints on model calculations at {\sqrts} = 13.6 TeV once the Run-III data for LHC becomes available.

==> table3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   This is a LaTeX file.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\documentclass[10pt]{article}
%\usepackage{multicol}
%\usepackage{graphicx}
%\usepackage{amsmath}
%\usepackage[a4paper]{geometry}
%\usepackage{rotating}

%\renewcommand{\baselinestretch}{1.05}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\setlength{\parindent}{.5cm} \setlength{\columnsep}{.5cm}
%\setlength{\oddsidemargin}{-.5cm} \setlength{\topmargin}{-1.5cm}
%\setlength{\textwidth}{17.5cm} \setlength{\textheight}{23.5cm}

%\begin{document}

\begin{table*}[!htb]\label{tab3}
{
\begin{center}
\caption{$K/\pi$ ratio at different energies, i.e., $\sqrt{s}$ = 6.3 GeV to 14 TeV by using simulations from various MC models along with the comparison of experimental values are displayed here.}
\small

\begin{tabular}{ccccccccccc}\\ \hline\hline
 Energy&DPMJET-III& EPOS1.99 & EPOS-LHC  &HIJING &Sibyll2.3d& QGSJET-II & Experimental  \\
 $\sqrt{s}$  &     & &&&& \\
\hline
    6.3  & 0.052$\pm$0.002 & 0.054$\pm$0.006 & 0.048$\pm$0.006& 0.062$\pm$0.023
 & ---- & 0.045$\pm$0.008&0.052$\pm$0.002\\
    17.3 & 0.087$\pm$0.003 & 0.084$\pm$0.008 & 0.077$\pm$0.007 & 0.095$\pm$0.014& 0.088$\pm$0.013 & 0.070$\pm$0.009 &0.082$\pm$0.003\\
    62.4 & 0.101$\pm$0.002 & 0.099$\pm$0.010 & 0.121$\pm$0.009 & 0.123$\pm$0.009 & 0.101$\pm$0.010 & 0.090$\pm$0.010 &0.094$\pm$0.002\\
    200 & 0.109$\pm$0.005 & 0.114$\pm$0.009 & 0.110$\pm$0.009 & 0.114$\pm$0.009 & 0.110$\pm$0.009 &0.126$\pm$0.009&0.103$\pm$0.008\\
    900 &  0.114$\pm$0.006 & 0.127$\pm$0.007 & 0.115$\pm$0.007 & 0.120$\pm$0.007  &  0.117$\pm$0.007 &0.137$\pm$0.007&0.123$\pm$0.004 \\
    2760 &  0.116$\pm$0.006 & 0.133$\pm$0.006 & 0.118$\pm$0.006 & 0.121$\pm$0.007 & 0.124$\pm$0.007 & 0.142$\pm$0.006&0.124$\pm$0.004\\
    7000 &  0.119$\pm$0.007 & 0.137$\pm$0.006 & 0.121$\pm$0.006 &  0.126$\pm$0.008 & 0.127$\pm$0.006& 0.143$\pm$0.006&0.124$\pm$0.005\\
    13000 & ----&  0.140$\pm$0.006 & 0.123$\pm$0.006 & 0.126$\pm$0.008
 &  0.129$\pm$0.006 & 0.144$\pm$0.005&----\\
    14000 & ---- &0.141$\pm$0.006 & 0.125$\pm$0.006 & 0.126$\pm$0.008 & 0.128$\pm$0.006 & 0.144$\pm$0.005 &----\\
\hline
\end{tabular}%
\end{center}}
\end{table*}

%\end{document}


==> table4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   This is a LaTeX file.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\documentclass[10pt]{article}
%\usepackage{multicol}
%\usepackage{graphicx}
%\usepackage{amsmath}
%\usepackage[a4paper]{geometry}
%\usepackage{rotating}

%\renewcommand{\baselinestretch}{1.05}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\setlength{\parindent}{.5cm} \setlength{\columnsep}{.5cm}
%\setlength{\oddsidemargin}{-.5cm} \setlength{\topmargin}{-1.5cm}
%\setlength{\textwidth}{17.5cm} \setlength{\textheight}{23.5cm}

%\begin{document}

\begin{table*}[!htb]
{
\begin{center}
\caption{Rapidity and {\ppt} ranges for different baryons studied}
\begin{tabular}{|c||c|c|c|c|c|}
\hline\hline
   $\sqrt{s}$ (TeV)&  $\overline{p}/p$ &  &  &\\
\hline\hline
 & DPMJET-III & PYHIA8  &  EPOS199 & EPOS-LHC  \\
\hline
       0.9&0.01763133&	0.006866&	0.0087296&	0.00207\\ 
\hline
    2.76 & 0.0195& 0.0104&	0.00989122&	0.006191  \\
\hline
     7 &0.032003&	0.017237&	0.01134&	0.008931 \\
 \hline
      & 0.016188	&0.01141&	0.0058767&	0.005932\\

   %  & $0.45 < p_T < 1.05$ GeV/$c$ & $0.5 < p_T < 4.0$ GeV/$c$ & $0.5 < p_T < 3.5$ GeV/$c$ \\
     %2.76   & $|y| < 0.5$   & $|y| < 0.8$    &  $|y| < 0.8$  \\
     %& $0.45 < p_T < 1.05$ GeV/$c$ & $0.5 < p_T < 4.5$ GeV/$c$ & $0.5 < p_T < 4.5$ GeV/$c$ \\
     %7   & $|y| < 0.5$   & $|y| < 0.8$    &  $|y| < 0.8$  \\
    % & $0.45 < p_T < 1.05$ GeV/$c$ & $0.5 < p_T < 10.5$ GeV/$c$ & $0.5 < p_T < 5.5$ GeV/$c$ \\
     %13.6   & $|y| < 0.5$   & $|y| < 0.8$    &  $|y| < 0.8$  \\
     %& $0.45 < p_T < 1.05$ GeV/$c$ & $0.5 < p_T < 10.5$ GeV/$c$ & $0.5 < p_T < 5.5$ GeV/$c$ \\
    
\hline
\end{tabular}
\label{tab1}
\end{center}}
\end{table*}

%\end{document}

